Hard to Cheat: A Turing Test based on Answering Questions about Images

Progress in language and image understanding by machines has sparkled the interest of the research community in more open-ended, holistic tasks, and refueled an old AI dream of building intelligent machines. We discuss a few prominent challenges that characterize such holistic tasks and argue for "question answering about images" as a particular appealing instance of such a holistic task. In particular, we point out that it is a version of a Turing Test that is likely to be more robust to over-interpretations and contrast it with tasks like grounding and generation of descriptions. Finally, we discuss tools to measure progress in this field.

==> concrete_challenges.tex <==
\section{DAQUAR: Building a Dataset for Visual Turing Challenge}
% 
DAQUAR \cite{malinowski14nips} is a challenging, large dataset for a question answering task based on real-world images. The images present real-world indoor scenes \cite{silbermanECCV12}, while the questions are unconstrained natural language sentences. DAQUAR's language scope is beyond the nouns or tuples that are typical to  recognition datasets \cite{ILSVRCarxiv14,rohrbach2011evaluating,LanYWM12}. Other, linguistically rich datasets either do not tackle images at all \cite{zelle1996learning,berant2013semantic} or consider only few in very constrained domain \cite{krishnamurthy2013jointly}, or are more suitable for the learning an embedding/image-sentence retrieval or language generation \cite{kong2014you,rashtchian2010collecting,rohrbach2012script,gong2014improving}. 
In this section we discuss in isolation different challenges reflected in DAQUAR. 
%\\
\paragraph{Vision and language}
The machine world in DAQUAR is represented as a set of images and questions about their content.
DAQUAR contains $1088$ different nouns in the question, $803$ in the answers, and $1586$ altogether (we use the Stanford POS Tagger \cite{toutanova2003feature} to extract the nouns from the questions).
If we consider only nouns in singular form in the questions, we still have $573$ categories.
The current state-of-the-art semantic segmentation methods on the NYU-Depth V2 dataset \cite{silbermanECCV12} can discriminate only between up to $37$ object categories \cite{gupta2014learning,lin2013holistic,gupta2013perceptual}, much fewer to what is needed. DAQUAR also contains other parts of speech where only colors and spatial prepositions are grounded in \cite{malinowski14nips}. 

Moreover, ambiguities naturally emerge due to fine grained categories that exist in DAQUAR.
For instance 'night stand', 'stool' and 'cabinet' sometimes refer to the same thing. There is also a variation in the naming of colors among the annotations. 
% Such ambiguities are tackled in \cite{malinowski14nips} using the multi-world approach.
% According to \cite{malinowski14nips} handling spatial reasoning is quite troublesome, and hand-crafted based approaches are doomed to fail in long run. Reference frame ambiguity is frequent in DAQUAR.
Questions rely heavily on the spatial concepts with different frame of reference.

DAQUAR includes various challenges related to natural language understanding.
% In particular the approaches that are based solely on the symbolic representation such as \cite{liang2013learning} are impractical in the long run as it is very difficult to define predicates for many phrases in DAQUAR - for instance already mentioned spatial predicates.
% On the other hand it is unclear if vector-based approaches can be used to ground the symbolic meaning with the perception.
Any semantic representation needs to work with the large number of predicates (reaching about $4$ million to account different interpretations of the external world), with questions of substantial length ($10.5$ words in average with variance $5.5$; the longest question has $30$ words), and possible language errors in the questions.

\paragraph{Common sense knowledge}
DAQUAR includes questions that can be reliably answered using common sense knowledge. For instance "Which object on the table is used for cutting?" already provides strong non-visual cues for the ``cutting'' object.
% , as the visual information on its own is ambiguous or even unnecessary.
Answers on other questions, such as "What is above the desk in front of scissors?", can be improved if the search space is reasonable restricted.
Moreover, some annotators hypothesize missing parts of the object based on their common sense. To sum up, we believe that common sense knowledge is an interesting venue to explore with DAQUAR. 

%"Which hand of the teacher is on her chin?", or "What is above the desk in front of scissors?". To quantify non-visual aspects of common sense knowledge in DAQUAR, we are collecting human answers who are instructed to answer on the questions without looking into the image. 

\paragraph{Question answering task}
The question answering task is also about understanding hidden intentions of the questioner with grounding as a sub-goal to solve. Some authors \cite{liang2013learning, berant2014semantic, malinowski14nips} treat the grounding (understood here as the logical representation of the meaning of the question) as a latent variable in the question answering task.
Others \cite{golland2010game} have modeled the pragmatic effects in the question answering task, but such approaches have never been shown to work in less constrained environments. 
